CORNET: Learning Table Formatting Rules By Example

Spreadsheets are widely used for table manipulation and presentation. Stylistic formatting of these tables is an important property for both presentation and analysis. As a result, popular spreadsheet software, such as Excel, supports automatically formatting tables based on rules. Unfortunately, writing such formatting rules can be challenging for users as it requires knowledge of the underlying rule language and data logic. We present CORNET, a system that tackles the novel problem of automatically learning such formatting rules from user examples in the form of formatted cells. CORNET takes inspiration from advances in inductive programming and combines symbolic rule enumeration with a neural ranker to learn conditional formatting rules. To motivate and evaluate our approach, we extracted tables with over 450K unique formatting rules from a corpus of over 1.8M real worksheets. Since we are the first to introduce conditional formatting, we compare CORNET to a wide range of symbolic and neural baselines adapted from related domains. Our results show that CORNET accurately learns rules across varying evaluation setups. Additionally, we show that CORNET finds shorter rules than those that a user has written and discovers rules in spreadsheets that users have manually formatted.

==> 2-introduction_backup.tex <==
\section{Introduction}

Spreadsheets are the most common table manipulation software, with around a billion monthly active users~\cite{spreadsheet-usage}.
Formatting is a fundamental and frequently used visual aid to better display, highlight or distinguish between data points in a spreadsheet.
By analyzing a large public spreadsheet corpus \cite{barik2015fuse,fisher2005euses} we found that close to 25\% of spreadsheets use some form of cell formatting to present data.

\emph{Conditional formatting} (CF) is a prominent feature that automates table formatting based on user-defined rules. It is available in all major spreadsheet manipulation tools like Microsoft Excel, Google Sheets, and Apple Numbers. All of them support predefined templates for popular rules, such as \emph{value greater than a specific value}. In Excel and Sheets, users can also author a custom boolean-valued formula to format cells. 

In this paper we present \system{}\footnote{\textbf{C}onditional \textbf{ORN}amentation by \textbf{E}xamples in \textbf{T}ables},
a system that allows users to automatically generate a formatting rule from examples in the form of formatted cells. \system{} takes a small number of user formatted cells as input to learn a highly likely formatting rule that generalizes to other cells in the column. For example, in Figure~\ref{fig:sample_ui}, after the user formats only two cells, \system{} is able to suggest the intended formatting rule without exposing the user to the underlying rule language. 

We believe that introducing the ability to automatically generate CF rules will be highly appreciated by spreadsheet users. Creating conditional formatting rules requires that users understand the syntax and logic behind conditional formatting, the
associated predefined templates, and potentially the overall formula language for more complex rules.
As of June 2022, more than 10,000 conditional formatting related questions were posted on the Excel tech help community alone  \cite{ExcelHelpForum}.
By analyzing the posts we discovered three key struggles that prevent users from using CF to its full potential.

\jose{This second part of this paragraph reads a bit risky to me: if we envision this, I think a reviewer can ask why not build it, like the aaai review we got}
Firstly, many users are unaware of the CF feature and manually apply formatting to their spreadsheets which is tedious and cumbersome. We envision an on-grid interaction for \system{} where we hand-raise and propose a CF rule as the user starts formatting their spreadsheet. 

Secondly, even if users are familiar with the feature they can struggle to introduce correct rules, resulting in erroneous formatting or no formatting. As \system{} produces only viable rules and 
\jose{again here: what preview? that seems to imply a UI}
shows a preview of the formatting we would apply, it will significantly lessen the users' debugging burden. Furthermore \system{} can efficiently update its suggestion with more examples as we will show in the evaluation section. \system{} is able to cover 15\% more cases when 2 examples are given instead of 1. \jose{I find it a bit odd to introduce a stat about learning scalability without first giving a top level number of how well we do overall}

Thirdly, we observe that authored rules can be either unnecessarily complex (the rules can be simplified to much shorter rules), or not generalizable (the rules may produce wrong formatting when the columns change or new values are added). As we show in the evaluation section, \system{} can produce rules that are significantly shorter in 60\% of cases
compared to rules that users write themselves when they employ custom formulas. 
\jose{another sentence here that starts to read like there is an UI}
\system{} can be re-run automatically with every change of the data and hand-raise when the rule should change based on the new data. 

We believe that some of the previously mentioned struggles can be reinforced by limitations in the interface used to apply conditional formatting. For example, navigating the CF UI in Excel can be challenging. Figure~\ref{fig:sample_ui} illustrates a real example of adding a CF Rule in Excel. For the case shown, it can be seen that the user has to navigate through multiple dialog boxes, make accurate selections and then write a formula in Excel's grammar to create the formatting rule. To add the rule shown in Figure-\ref{fig:sample_ui}, a user would need to make 7 interactions (click or type) in Excel and Apple Numbers and 8 in Google Sheets.  
In contrast, \system{} is able to learn this rule with 2 formatted examples without the user knowing about the underlying rule language. \jose{do we need to make this claim on producitivty? we can't substantiate it yet and I don't feel it adds much -- I would cut the rest of this paragraph}We believe this automated learning will improve the users' productivity. This is particularly important as we found that the templates are not sufficiently diverse - even using logical operations like \textsc{or} and \textsc{and} requires writing custom formulas. As \system{} automatically generates the rule user would not have to learn to write custom formulas.

\jose{I think we should move this up when discussing issues with the current CF systems -- right now we discuss some challenges, then jump to how cornet helps, and then jump back again to issues -- which I find confusing.}
Additionally, there is no validation for data types, which can cause surprising results, for example, it is possible to write a rule that formats cells whose value is \emph{less than 5} for a text column. \system{} uses type information and will not suggest such erroneous rules. 

% In this paper we propose a system that takes away the brunt of the formatting work away from the users and abstracts it in a way that the user can directly convey their 
% \mr{"their" maybe? not sure what strategy we want here but should be consistent throughout} 
% intent via formatting few cells that the system then uses to come up with accurate formatting rules on the user's behalf. We focus on rule based formatting in Excel which is one of the most popular tool for manipulating tabular data.
% \gust{This paragraph needs some more citable sources.}
%
% Excel is the most popular tool for manipulating tabular data. Spreadsheets in Excel are a great visual tool for understanding and sharing data, with formatting being one of the most basic visual aids. \mr{I think we can position our contribution much more generally - CF seems to be a common concept in many spreadsheet tools (e.g. google sheets, apple numbers, etc). So maybe we can say: spreadsheets are most common table manipulation software, and CF is common concept in spreadsheet tools (excel, google, apple ...). In this paper we focus on CF in Excel which is most used spreadsheet tool} 
% 
% \jose{do we need to say this so early on? Can we say we are inspired by Excel, but the approach is general}
% Excel is one of the most popular spreadsheet engines which supports conditional formatting.
% Excel supports Conditional Formatting (CF), using which users can define rules over a selection of cells to format them.
% CF in Excel aims to automate spreadsheet formatting and also leave an audit trail for users to review the rules at a later point in time.

% Figure~\ref{fig:excel_cf_ui} illustrates the process of adding a new conditional formatting rule in Excel, where the user wants to highlight only those cells in the column that contain the string \textit{``(SR)''} by using a predefined template.

% \vule{I think we are going back and forth between CF and its problem.
% We can merge this paragraph with the first paragraph and move the sentences after ``Unfortunately..'' to this paragraph. The flow then becomes ``Spreadsheet popular $\rightarrow$ CF is important $\rightarrow$ CF has challenges''.
% Also, while I think Figure 1 is useful, it doesn't add much to the paper flow.
% What are the points we are trying to make it with it? Originally we intended to say that this design may lead to bad predicates, but I don't see it here.}

% \begin{figure}[t]
% \centering
% \includegraphics[width=\columnwidth]{Images/intro.png}
% \caption{Interface for adding a new CF rule in Excel. The user \circled{\textbf{1}} selects a range of cells which they want to format, \circled{\textbf{2}} selects the conditional formatting option in the styles menu and selects new rule,  and \circled{\textbf{3}} selects the type, sub-type, arguments and  desired formatting of the rule. \circled{\textbf{4}} Excel generates a rule for the formatting}
% \label{fig:excel_cf_ui}
% \end{figure}

%that will be evaluated for each cell.
% \gust{What is the difference between rule-based and conditional formatting? Perhaps just call it conditional formatting from the start and split part of previous paragraph off to this one.}
% To add a conditional formatting rule in Excel, a user can select the feature from the styles section in the home pane. This opens a dialog box where the user can choose to create a rule from pre-defined templates or define a rule based on a custom function. 
% Figure~\ref{fig:excel_cf_ui} illustrates the process to add a new CF rule in Excel where The user wants to highlight only those cells in the column that contain the string \textit{``(SR)''}.
% To accomplish this, the user first selects the column which they want to format over, next they head over to the conditional formatting option located in the styles section of the Home pane. This opens a CF drop-down menu where the user can select the option to add a new rule. This launches the CF dialog box where the user can choose to select from predefined rule templates or write a custom rule. 
% In this case the user chooses the \textit{"Format cells that contain"} template.
% Once the user selects a template, they need to select the sub-type of the rule and provide arguments for the rule.
% The user chooses the rule type as \textit{"Contains Text"} and specifies the argument as \textit{"(SR)"}. 
% Once the rule selection is done, the user then defines the formatting he wants the rule to apply. In this case, the user chooses a solid green cell fill colour. Figure~1 (4) also shows the formula Excel generates for this template based CF rule.
% \mr{Good to have this figure, but description seems too abstract: describe what exactly the user's intent is in this case and the logic required (they want to highlight only those cells that contain ...). Also show the generated formula in Excel and what it means (as you refer to an excel formula in figure 2 and users may have less context about it). Also, maybe use a scenario where rule is not too simple (in this case it just seems like highlighting cells that have a fixed value? maybe a "string contains" example would be interesting enough)}
% -- Rewrote and updated the figure
% \gust{A lot of overlap between this paragraph and caption. I suggest keeping the description in the caption and just briefly mention it here, possibly integrating with another paragraph.}

% \jose{this can be merged earlier when introducing the problem -- this is inline with Vu's feedback above}
% Conditional formatting is a powerful feature, but this makes it more difficult to navigate for users.
% Even for more experienced users---who can write accurate rules---the process is tedious and requires effort.
% Firstly, creating conditional formatting rules requires that users understand the syntax and logic behind conditional formatting, the
% associated predefined templates, and potentially the overall formula language for more complex rules.
% As of June 2022, more than 10,000 conditional formatting related questions were posted on the Excel tech help community alone  \cite{ExcelHelpForum}.
% By analyzing the posts we discovered three key struggles that prevent users from using CF to its full potential.
% First, many users are unaware of this feature and manually apply formatting to their spreadsheets which is tedious and cumbersome. 
% \jose{we don't address this first concern in our work, should we remove this? or clarify scope} -- we have an RQ for this now
% Second, when a user does know about CF and tries to enter a CF rule, they sometimes fail to do so correctly resulting in erroneous formatting or no formatting. The users then eventually end up ignoring CF and manually formatting the sheet.
% Third, even when users are able to navigate and write valid CF rules that correctly matches their desired formatting, the rules are either unnecessarily complex (can be rewritten to much simpler rules), or not generalizable (may produce wrong formatting when the columns change or new values are added).
% \begin{example}
% Figure~\ref{fig:inccorect_cf} shows a case from a public spreadsheet where the user tried to use conditional formatting, but was unable to write the correct rule and then had to manually format the sheet.
% They wanted to highlight all cells with a value greater than or equal to 50.
% Their rule, however, evaluates to false in all cases, because they compared the value of a particular cell (E9) instead of the intended range.
% \end{example}

% \begin{example}\gust{Remove Figure 2 and keep relevant information in the example only.}
% Figure~\ref{fig:inccorect_cf} shows a case from a public spreadsheet where the user wanted to highlight cells with value $< 5$, but wrote an incorrect rule and had to manually format the sheet.
% % F9 < "5"
% \end{example}

\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{Images/motivating_ex.png}
\caption{Adding a CF Rule in Excel: \circled{1} CF Option in Styles Pane; \circled{2} CF Dropdown Menu to add new rule \circled{3} CF New Rule Dialog box; \circled{4} Resulting formatted column from rule.  After the user formats two cells, \system{} automatically suggest the intended CF rule for the user.}
\label{fig:sample_ui}
\end{figure}

% \mr{Start with user's desired intent: The user wants to highlight all cells with value less than 85. However, the rule he creates ...} -- Rewritten
% The user then manually formatted the entire sheet coloring cells that have value greater than equal to 50, which is effort that could have been saved had the user been able to write the rule accurately.
% \mr{is this a real example of a user? if so, would be good to state that and where its from (like telemetry or help forum, etc)} -- Added that it is from telemetry where the figure is first cited
% The formatting that the user desired needed a simple cell value greater than equal rule but due to the in-expertise of the users these simple cases are also challenging to handle.
% \gust{I would put this example in an explicit example environment.}

% \carina{we are not addressing the UI in the paper so is it worth spending so much space on it?}
% \gust{I \emph{thought} that we addressed difficulties with the UI because with our system, users don't need the UI.}
% Some of these struggles are reinforced by limitations in the interface used to apply conditional formatting. For example, using logical operations like \textsc{or} and \textsc{and} requires writing custom formulas. Additionally, there is no validation for data types, which can cause surprising results, for example, it is possible to write a rule that formats cells whose value is \emph{less than 5} for a text column.
% \todo{discoverability scoping}

% which causes formatting based on Excel’s string to integer casting.
% An automated rule learning system can help the users in all the three cases listed above by suggesting rules to users as they are formatting their spreadsheets, ensuring correctness of rules, and saving the effort to write a rule by automatically learning one.
% First, as highlighted in Figure~\ref{fig:excel_cf_ui}, the process of adding a new CF rule is tedious and might become challenging to navigate.\gust{Isn't this case covered by the previous paragraph?}
% 
% \jose{this paragraph feels like pandering to Excel -- I also think the point of difficulty has been made, this can probably be removed, so we can merge this with prior text and reference figure there if helpful}
% Thus, \gust{This sentence captures the gist of the paragraph---put it as the first sentence.}

% \mr{a bit of repetition and back and forth in the previous two paragraphs: maybe start with high level points about Excel and the difficulties with CF, then illustrate these difficulties with the concrete example from Figure 2} -- Rewritten

% \jose{emphasize that they annotate few examples}
% In this paper we present \system{} (\textbf{C}onditional \textbf{ORN}amentation by \textbf{E}xamples in \textbf{T}ables),
% a system that allows users to automatically generate a formatting rule from examples in the form of formatted cells, thus overcoming the challenges outlined. \system{} takes a small number of user formatted cells as input to learn the most likely formatting rule that generalizes to other cells in the column.
% \system{} explores possible predicates for the target column, hypothesizes cell grouping via semi-supervised clustering and then learns candidate rules by employing an iterative tree learning procedure. Since multiple rules may match the examples, \system{} uses a neural ranker to return the most likely CF rule to the user.
% For example, in Fig.~\ref{fig:sample_ui}, after the user formats only two cells, \system{} is able to suggest the intended CF rule without exposing the user to the underlying rule language.


To solve the task of learning conditional formatting rules \system{} explores possible predicates for the target column, hypothesizes cell grouping via semi-supervised clustering and then learns candidate rules by employing an iterative tree learning procedure. Since multiple rules may match the examples, \system{} uses a neural ranker to return the most likely CF rule to the user.

Traditional programming-by-example (PBE) systems~\cite{flashfill, flashextract} can typically derive
useful search constraints by relating properties of the outputs to the inputs provided (e.g. an output text may share spans with an input text).
This is challenging to do in CF learning as the user only provides what amounts to a small number of formatting labels.
Recent PBE works like \cite{morpheus-pbe, chen-wang-pbe, scythe-pbe} use richer signals in the form of output examples or user interaction to navigate the search space and disambiguate programs.
The predicate generation and clustering step in \system{} mitigates this by generating and applying
simple predicates, which jointly can help \emph{hypothesize} such formatting labels for the entire target column.

Once these hypothesized labels are available, we can apply our iterative rule enumeration procedure.
Much like other PBE problems, we enumerate multiple possible programs consistent with our
hypothesized outputs. Our enumeration uses tree learning as we can easily
enforce consistency over user-provided examples. The learning process is iterative to generate diverse rules. Finally, we employ a ranker that can disambiguate between
these competing programs by capturing properties not just of the rule but also of the
underlying data and the execution of the rule on that data.
%\system{} is general and can support any tabular data engine that has rule-based formatting. 

%\system{} is the first programming by example system that focuses on predicting a likely output first and then learning rules that approximate this output. This is crucial because the learning dimension of formatting rules is very high, and often requires too many examples to learn a rule. We instead observe that the output space is much smaller than the program space in our setting, and we use this intuition to design an output-first synthesis procedure.

% \begin{figure}[htb]
% \centering
% \includegraphics[width=0.85\columnwidth]{Images/incorrect_rule.png}
% \caption{Example of incorrectly using CF: \circled{1} a user defined a custom rule that always evaluates to false (it compares the cell to the string ``5'' instead of the number 5); \circled{2} because the rule does not format any cell, the user had to manually format the sheet; \circled{3} the correct rule for the formatting.} 
% % \gust{So the CF rule from (2) is not applied?} -- No
% \label{fig:inccorect_cf}
% \end{figure}

% Referring back to Figure~\ref{fig:excel_cf_ui}, with \system{} the user can simply format the first and third cell in the column and \system{} intelligently learns the desired CF rule.
% \vule{Here we should clarify refer to Example 1 to show that CORNET can help with the scenario. We may include a small screenshot of the suggestion to close the imagination gap.}
% \system{} uses a custom grammar to define, instantiate and enumerate CF Rules. A set of predicates, based on the grammar, is generated symbolically for the input spreadsheet. The system clusters the column cells constrained on the positive formatted examples from the user and enumerates multiple rules over the predicate set using the clustered labels. Finally, a neural ranker scores these candidate rules and we get the final set of learned rules.

% \jose{the introduction is missing a paragraph summarizing our experimental results -- we should mention briefly the benchmarks, baselines, and main takeaways}

To evaluate \system{}, we created a benchmark of 105K real user tasks from public Excel spreadsheets. \system{} can learn CF rules from as few as two examples and outperforms existing and custom symbolic and neural baselines that were adapted for this task.

% The goal for this research is to create a general system that can learn formatting rules based on few examples from the user.
This paper makes the following key contributions:
\begin{itemize}
    \item Based on the observation that users often struggle to format their tabular data, we introduce the novel problem of learning conditional formatting rules from examples.
    \item We propose \system{}, a system
    that learns CF rules from examples over tabular data.
    % \system{} is based on a novel PBE methodology that leverages few examples to predict more examples and then generalize them into an intended CF rule. This is done via a novel combination of symbolic (predicate set) enumeration, ML methods for semi-supervised clustering (to predict more examples using predicate set) and iterative tree learning (to propose candidate rules), and a neural ranker (to pick an intended rule). \todo{shorten this}
    \item We create a dataset of 105K real formatting tasks extracted from public spreadsheets. We release this dataset to encourage future research.
    \item We evaluate \system{} extensively on existing and custom baselines and show that it outperforms both symbolic and neural baselines by \todo{XX\%} on our benchmark.
    % \jose{on XXX real use spreadsheets}
    % \jose{I'm not clear on this last contribution -- can we just say as: We perform an extensive experimental evaluation comparing to XYZ}
    % \item We perform an extensive experimental evaluation comparing \system{} to popular neural and symbolic systems.
\end{itemize}

% \jose{this sentence below feels out of place and sounds like we're putting down the problem of CF itself slightly} -- agree. tried to rephrase
% \system{} aims to effectively address the problem of learning CF rules automatically for users but the learning paradigm is extendable to problems beyond the scope of formatting. \system{} is the preliminary step to performing various other sophisticated analysis such as conditional transformations for data cleaning, filtering, validation or visualizations. Our work on automating conditional formatting rules shall motivate research in automating other such encompassing workflows. 
% \todo{remove}

